Consistent Variance Estimation for Q-Function Estimators in Finite-Horizon MDP Tree Search

We study the variance of Q-function estimators in finite-horizon, finite-state Markov decision process (MDP) tree search. We show that the variance decomposes into three components attributed to the immediate reward collected, probabilistic state transitions, and uncertainty in future state value function estimates. Using this decomposition, we show that the sample variance estimator based on the assumption of i.i.d. paths is biased, underestimating the true variance, and the bias does not vanish in the limit. We then propose a recursive variance estimator that is consistent. To enable efficient storage and computation, we derive an equivalent implementation of the recursive estimator using only node-local statistics that can be iteratively updated. This consistent variance estimator is integrated into two Monte Carlo Tree Search (MCTS) sampling procedures for finite-horizon MDPs. In numerical examples from inventory control and kidney paired donation matching, the new estimator improves the performance of the MCTS algorithm relative to a baseline that uses the i.i.d.-based sample variance estimator.

==> old_intro.tex <==
\section{Introduction}
\label{sec:introduction}
\IEEEPARstart{W}{e} consider a sequential decision-making problem in which an agent interacts with an environment modeled as a finite-horizon Markov decision process (MDP). At each step, the agent observes the state of the system, selects an action, receives a reward, and the system transitions to a new state. The reward is typically stochastic, with its distribution depending on the agent's current state, the action taken, and the resulting next state. Transition probabilities are determined by the current state and the chosen action. The objective is to identify the optimal action for any initial state of the MDP that maximizes the expected total reward over the entire horizon. We evaluate the decision policy based on the probability of correctly selecting the best action at the initial stage of the MDP.

In this paper, we focus on Monte Carlo Tree Search (MCTS) \cite{fu2024tutorial} as the solution method. Compared to other solution methods such as dynamic programming, MCTS has several notable advantages. MCTS samples MDP trajectories and performs a depth-first search of the decision tree to focus computational effort on the most promising parts of the decision space. Therefore, MCTS does not require full knowledge of transition probabilities or reward distributions. MCTS performs effectively for problems with a high-dimensional state-decision space and complex environments. It progressively refines estimates as more simulations are executed and improves decision-making quality over time, making it suitable for time-constrained decision-making. Thanks to these strengths, MCTS has many notable successes in domains such as inventory management \cite{preil2022artificial}, path planning \cite{qian2022path}, and combinatorial games, with Google DeepMind's AlphaGo program being the most famous case \cite{silver2016mastering}. 

%Similar to tabular Q-learning method, MCTS does not assume that the agent has perfect information about the environment. In contrast, if the distributions and dynamics of the environment are known, the optimal action can be determined using dynamic programming. MCTS performs a depth-first tree search with an adaptive algorithm, such like multi-armed bandit (MAB) model-based upper confidence bound (UCB), leading to the Upper Confidence Tree (UCT). MCTS has been extensively developed and applied to various games such as Othello and Go. To address different types of problems, several variations of MCTS have been introduced, including flat UCB (and its extension, the bandit algorithm for smooth trees) and single-player MCTS (for single-player games).

A generic MCTS algorithm has four main steps as illustrated in Figure~\ref{fig:mcts}: \emph{selection, expansion, simulation}, and \emph{backpropagation}. \emph{Selection} refers to iteratively choosing an action at a non-leaf node as MCTS executes a new iteration and traverses down the current grown decision tree to a leaf node. Upon reaching a leaf node, the \emph{expansion} step expands the leaf node by exploring available actions and reachable states. The \emph{simulation} (also known as \emph{roll-out}) step then estimates the value of the new states by collecting rewards up to a given node, which could correspond to the actual end of the horizon, or simply to a point where the current estimation may be considered sufficiently accurate so as not to require further simulation. The \emph{backpropagation} (also known as \emph{backup}) step returns the leaf value estimated by the simulation step to update nodes closer to the root.
\begin{figure}[htbp]
\centering
  \includegraphics[width=0.5\textwidth]{images/mctsframework.png}
  \caption{An illustration of key steps during an MCTS iteration.}
  \label{fig:mcts}
\end{figure}

Among these four steps, \emph{expansion} is straightforward and \emph{simulation} is highly problem-dependent. This paper focuses on how to perform the \emph{selection} and \emph{backpropagation} steps. Algorithms for these two steps can be applied across diverse MCTS applications have a fundamental impact on the quality of the decision made by an MCTS with a limited computing budget. As will be elaborated later in this paper, these two steps are also closely intertwined and need to be addressed together. 

AlphaGo uses a selection policy based on the well-known upper confidence bound for trees (UCT) policy \cite{silver2016mastering}, which is closely related to the adaptive multistage sampling (AMS) algorithm for MDP \cite{chang2005adaptive}. UCT selects the action that has the highest state-action value ($Q$ function) plus an exploration term, which is calculated using the number of visits to the state-action pair. The backpropagation step updates the $Q$ function value as the updated sample average of the simulation outcome. The UCT policy is based on the upper confidence bound (UCB) policy derived originally for minimizing the cumulative regret in a canonical multi-armed bandit (MAB) setting \cite{auer2002finite}. However, the cumulative regret objective function is a misfit for finite-horizon MDP, where the objective is to select the best action that leads to the best outcome at the end of the horizon, e.g., to win a Go game. A new formulation is proposed by \cite{chen2000simulation} to maximize the probability of selecting the best action, and implemented by \cite{li2022optimal} onto the MCTS problem. The new formulation, referred to as optimal computing budget allocation (OCBA), considers both the mean and variance in the $Q$ function estimate to determine the allocation. The new OCBA selection policy was shown to outperform UCT policy in several finite-horizon MDP problems \cite{li2022optimal}. An MCTS-OCBA Othello program is then shown to outperform an MCTS-UCT Othello program in \cite{fu2024tutorial}. 

While the new OCBA policy is shown to be a promising selection policy for solving general finite-horizon MDP problems using MCTS, the work of \cite{li2022optimal} did not address how the variance of $Q$ function should be updated during the backpropagation step. A simplifying assumption was made to regard back-propagated value as independent and identically distributed (i.i.d.) samples and the sample variance is then calculated. As we shall elaborate, these samples are not i.i.d. and using the sample variance may significantly underestimate the true variance in $Q$ function value estimate. In this paper, we tackle this problem and propose new methods to properly estimate the variance in $Q$ function value estimates for use in an OCBA selection policy. Furthermore, we show how the backpropagation step needs to be improved to provide the information needed by the new variance estimator. 

%We focus on trees storing means and variances and using them for its selection decisions. Quantifying uncertainties such like variances is important in MCTS, as most selection algorithms, such as Upper Confidence Bound (UCB) and Optimal Computing Budget Allocation (OCBA), rely on uncertainties to make their budget allocations. OCBA is our focus since its uncertainty measure is the estimated variance of the sample mean, while UCB uses a confidence interval based on Hoeffding's inequality. Generally speaking, actions with higher estimated values or estimated variances requires more samples. For non-trivial MDPs and their Monte Carlo Trees, uncertainties accumulate throughout the MDP structure, passing across time. In this paper, we will analyze this variance and derive a OCBA algorithm extendable to MDP problems (we call it look-forward OCBA, LFOCBA).

The literature on the analysis of variance in simulation-based MDP value estimates is limited. In \cite{mannor_tsitsiklis_2011}, the mean and variance of the cumulative rewards of an MDP are analyzed. Sobel \cite{c61e0c2e-17aa-3604-8b99-64bae6cd8009, sobel1994meanvariance} derived a variance formula for MDPs in a time-homogeneous, discounted infinite-horizon environment. Our work extends the MDP literature by deriving results in a general finite-horizon MDP setting. In addition, our results apply to both the cumulative reward and the reward estimators at each stage, generating additional insights and providing the additional information needed to derive an efficient estimator of the variance for use in OCBA-type of selection policies.

%We focus our effort on the finite-state, finite-action setting, since the continuous state space problem is theoretically complex, and requires a value approximation method such as artificial neural networks \cite{li_ML}. 

%We build upon an idea presented in the OCBA-MCTS \cite{li2022optimal} algorithm and improve upon it. We seek to improve the OCBA-MCTS algorithm in two aspects: to derive a variance formula for an MDP and a Monte Carlo Tree, and to find an efficient estimator for this variance.

In the rest of the paper, we first present the formulation and derive the main theorem of this paper in Section \ref{sec:variance}. %, decomposing the variance of the value estimator $\hat{Q}$ into a current-period component and a future-period component.
In Section \ref{sec:consistent}, we present the new variance estimator and establish its consistency. %show that the new variance estimator is consistent and propose a recursively-defined consistent estimator that's a sum of the sample variance estimator and a probability-discounted next-period variance estimator. 
Section \ref{sec:efficient} discusses how the backpropagation step needs to be revised. %to provide the information needed for the new consistent variance estimator. This leads us to use a set of sufficient and consistent variance estimators that decouples the rewards and the future state values, leading to an efficient updating rule. 
In Section \ref{sec:LFOCBA}, we derive a version of the OCBA based on the result in the previous section and present our new algorithm. Section \ref{sec:examples} presents numerical results on two case studies. We conclude the paper in Section~\ref{sec:conclusion}. %, we tested the algorithm on a few MDP problems in inventory control and kidney paired donation. Our results shows the sufficient estimators improves the sampling efficiencies by a lot. The consistent variance estimation further improves on some problems but has no effect on other problems compared to the biased variance estimation.

